Learning the score under shape constraints

Score estimation has recently emerged as a key modern statistical challenge, due to its pivotal role in generative modelling via diffusion models. Moreover, it is an essential ingredient in a new approach to linear regression via convex $M$-estimation, where the corresponding error densities are projected onto the log-concave class. Motivated by these applications, we study the minimax risk of score estimation with respect to squared $L^2(P_0)$-loss, where $P_0$ denotes an underlying log-concave distribution on $\mathbb{R}$. Such distributions have decreasing score functions, but on its own, this shape constraint is insufficient to guarantee a finite minimax risk. We therefore define subclasses of log-concave densities that capture two fundamental aspects of the estimation problem. First, we establish the crucial impact of tail behaviour on score estimation by determining the minimax rate over a class of log-concave densities whose score function exhibits controlled growth relative to the quantile levels. Second, we explore the interplay between smoothness and log-concavity by considering the class of log-concave densities with a scale restriction and a $(\beta,L)$-H\"older assumption on the log-density for some $\beta \in [1,2]$. We show that the minimax risk over this latter class is of order $L^{2/(2\beta+1)}n^{-\beta/(2\beta+1)}$ up to poly-logarithmic factors, where $n$ denotes the sample size. When $\beta < 2$, this rate is faster than could be obtained under either the shape constraint or the smoothness assumption alone. Our upper bounds are attained by a locally adaptive, multiscale estimator constructed from a uniform confidence band for the score function. This study highlights intriguing differences between the score estimation and density estimation problems over this shape-constrained class.

==> macros.tex <==
% --- Packages -----

% Maths packages
\usepackage{amsmath,amssymb,amsfonts,amsthm,lipsum}
\usepackage{amscd}
\usepackage{bbm,bm} 
\usepackage{cases}
\usepackage[mathscr]{euscript}

% Packages for references and links
\usepackage{breakcites}
\usepackage{natbib}
% hypertexnames: see the supplementary material and  https://bit.ly/2UwcJfo and https://bit.ly/2RLQVuk
\RequirePackage[colorlinks,citecolor={blue!60!black},urlcolor={blue!70!black},linkcolor={red!60!black},breaklinks,hypertexnames=false]{hyperref}
\usepackage[norefs,nocites]{refcheck}

% Packages for formatting, layout and diagrams
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{array}
\usepackage[small]{caption}
\usepackage{epic,eepic, epsfig, psfrag}
\usepackage{enumerate}
\usepackage{fullpage}
\usepackage{graphicx}
\usepackage[sf,bf,SF,footnotesize]{subfigure}
\usepackage{setspace}
\usepackage{tikz}
\usepackage{xcolor}
\usepackage{comment}

% Packages for macros
\usepackage{etoolbox}

% ----- Layout parameters -----

% Page Layout
% \setlength{\textheight}{23.4cm}
% \setlength{\topmargin}{-0.15in}
% \setlength{\footskip}{36pt}
\usepackage[margin=1in]{geometry}

% ----- Layout commands -----

% Colours 
\newcommand{\teal}[1]{{\color{teal}#1}}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\orange}[1]{{\color{orange}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\purple}[1]{{\color{purple}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}

\newcommand{\purplesout}[1]{{\color{purple} \sout{#1}}}

% ----- Mathematics -----

% Mathematics environments
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem*{remark*}{Remark}

% Mathematics format/layout
\def\mathbi#1{\textbf{\em #1}}

% Common symbols and operators
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Ind}{\mathbbm{1}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\norm}[1]{\|{#1}\|}
\newcommand{\ipr}[2]{\langle #1, #2 \rangle}

\DeclareMathOperator\Var{Var}
\DeclareMathOperator\Cov{Cov}
\DeclareMathOperator\tr{tr}
\DeclareMathOperator*{\arginf}{arginf}
\DeclareMathOperator*{\argsup}{argsup}
%\newcommand{\argmax}{\text{argmax}}
%\newcommand{\argmin}{\text{argmin}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\sargmin}{sargmin}
\DeclareMathOperator*{\sargmax}{sargmax}
\DeclareMathOperator*{\sgn}{sgn}
\DeclareMathOperator*{\essinf}{essinf}
\DeclareMathOperator{\supp}{supp}

\newcommand{\functionClassUnimodal}{\Phi_{\mathrm{uni}}}

\newcommand{\E}{\mathbb{E}}
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\iid}{\overset{\mathrm{iid}}{\sim}}
\newcommand{\cvas}{\overset{a.s.}{\to}}
\newcommand{\cvp}{\overset{p}{\to}}
\newcommand{\cvd}{\overset{d}{\to}}
\newcommand{\eqd}{\overset{d}{=}}
\newcommand{\indep}{\mathrel{\perp\!\!\!\perp}}

\DeclareMathOperator\TV{TV}
\DeclareMathOperator\dhell{H}
\DeclareMathOperator\KL{KL}
\newcommand{\kullbackLeibler}{\mathrm{kl}}
\newcommand{\laplaced}{\,\mathrm{d}}
\newcommand{\lebesgue}{\mathcal{L}}

\newcommand{\X}{\mathcal{X}}

\newcommand{\populationUncertainty}{\mathrm{U}_{n,\delta}}
\newcommand{\empiricalUncertainty}{\widehat{\mathrm{U}}_{n,\delta}}

\newcommand{\rhoByNDelta}{\rho_{n,\delta}}

\newcommand{\fLevelSet}{A(\epsilon)}
\newcommand{\fLevelSetBound}[1][\omega]{a_{\epsilon,#1}}
\newcommand{\fLevelSetLower}{\fLevelSetBound[-1]}
\newcommand{\fLevelSetUpper}{\fLevelSetBound[1]}
%\newcommand{\fLevelSetLower}{a_{\epsilon,-1}}
%\newcommand{\fLevelSetUpper}{a_{\epsilon,1}}
\newcommand{\bulkInterval}{\mathcal{I}}
\newcommand{\support}{\mathrm{supp}(f_0)}
\newcommand{\clsupport}{\mathrm{Cl}(\support)}

\usepackage[normalem]{ulem}

\newcommand{\empiricalProb}[1][n]{\Prob_{#1}}
\newcommand{\probDistribution}{P_0}
\newcommand{\epsilonByNDeltaMod}{\epsilon_{n,\delta}}
\newcommand{\epsilonByNDeltaModPrime}{\nu_{n,\delta\red{,\beta,L}}}
\newcommand{\etaByNDeltaMod}{\eta_{n,\delta,\beta\red{,L}}}
\newcommand{\epsilonByNDeltaModr}[1][]{\varepsilon_{n,\delta \red{,f_0}{#1}}}
\newcommand{\epsilonByNDeltaPlus}{\varepsilon_{n,\delta}^+}
\newcommand{\ratioEpsilonOverP}[1][\varphi]{\rho_{#1}}

\newcommand{\avgDerivSignNoArg}{\hat{\tau}}
\newcommand{\avgDerivSign}[2]{\avgDerivSignNoArg_{#1,#2}}


\newcommand{\scoreConfidenceBoundByBandwidthWidth}{\hat{V}_{n,\delta,h}}

\newcommand{\scoreMagnitudeConfidenceBoundByBandwidthCentre}[1][\omega]{\hat{M}_{n,\delta,h}^{(#1)}}

\newcommand{\scoreConfidenceBoundByBandwidthCentreDenominator}[1][\omega]{\hat{D}_{n,\delta,h}^{(#1)}}

\newcommand{\scoreConfidenceBoundByBandwidthCentreMagnitude}[1][\omega]{|\hat{\psi}|_{n,\delta,h}^{(#1)}}

\newcommand{\scoreConfidenceBoundByBandwidthCentreMagnitudeNumerator}[1][\omega]{\hat{M}_{n,\delta,h}^{(#1)}}

\newcommand{\scoreConfidenceBoundSetOfBandwidths}{\hat{\mathrm{H}}_{n,\delta}}

\newcommand{\scoreConfidenceBoundByBandwidthCentre}[1][\omega]{\hat{\psi}_{n,\delta,h}^{(#1)}}
\newcommand{\scoreConfidenceBoundShapeConstrained}[1][\omega]{\hat{\psi}_{n,\delta}^{(#1)}}
\newcommand{\scoreEstimateShapeConstrained}{\hat{\psi}_{n,\delta}}

\newcommand{\kernelFunction}[1][]{K_{#1}}
\newcommand{\goodEvent}{\mathcal{G}_{n,\delta}}

\newcommand{\holderExponentLogDensity}{\beta}
\newcommand{\holderExponentScore}{\zeta}

\newcommand{\popScore}[1][]{\psi_0}
\newcommand{\popScoreN}[1][]{\psi_0^{(#1)}}

\newcommand{\distributionMode}{m_{f_0}}
\newcommand{\localScoreErrorRate}[1][\omega]{\Delta^{#1}_\psi}
\newcommand{\hMax}{h_{\infty}}

\newcommand{\setOfBandwidthsByPoint}[1][\omega]{\mathcal{H}^{#1}_{f_0}}

\newcommand{\setOfBoundingPairs}[1][\omega]{\mathcal{Q}^{#1}_{f_0}}

\newcommand{\JLo}{J_\mathrm{L}(n,\delta)}
\newcommand{\JHi}{J_\mathrm{U}(n,\delta)}
\newcommand{\hj}{\red{\mathring{h}}}


\newcommand{\totalVariationExponent}{\gamma}
\newcommand{\totalVariation}{\mathrm{V}_{\totalVariationExponent}}
\newcommand{\localHolderConstant}{\zeta_{f,\totalVariationExponent}}
\newcommand{\lebesgueMeasure}{\lambda}

\newcommand{\COneZH}{\Pi_{1,z,h}}
\newcommand{\CTwoZH}{\Pi_{2,z,h}}
